EventNet: Asynchronous Recursive Event Processing

Event cameras are bio-inspired vision sensors that mimic retinas to asynchronously report per-pixel intensity changes rather than outputting an actual intensity image at regular intervals. This new paradigm of image sensor offers significant potential advantages; namely, sparse and non-redundant data representation. Unfortunately, however, most of the existing artificial neural network architectures, such as a CNN, require dense synchronous input data, and therefore, cannot make use of the sparseness of the data. We propose EventNet, a neural network designed for real-time processing of asynchronous event streams in a recursive and event-wise manner. EventNet models dependence of the output on tens of thousands of causal events recursively using a novel temporal coding scheme. As a result, at inference time, our network operates in an event-wise manner that is realized with very few sum-of-the-product operations---look-up table and temporal feature aggregation---which enables processing of 1 mega or more events per second on standard CPU. In experiments using real data, we demonstrated the real-time performance and robustness of our framework.

==> fig/_batch_detail.tex <==
\begin{figure}[!h]
\includegraphics[width=1\columnwidth]{fig/batch_detail.pdf}
\caption{
\label{fig:batch_detail}
\textbf{Mini-batch composition.}
Using a random sample event stream $\mathbf{e}_i$, a single batch is composed by concatenating each stream into batch dimension.
See also the explanation on \Fig 3 with the main article.
}
\end{figure}

==> table/accuracywindow.tex <==
\begin{table}
\caption{\label{table:accuracywindow}$\textbf{The effects of time window on ETHTED+.}$
Comparison of performance of our EventNet and  PointNet using different time window is shown.
}
\begin{center}

\begin{tabular}{cc|c}
\hline 
\multicolumn{2}{c|}{} & \multicolumn{1}{c}{ETHTED}\tabularnewline
\cline{3-3} 
\multicolumn{2}{c|}{} & Object-motion \tabularnewline
\cline{3-3} 
 & Window size $\tau${[}ms{]} & error {[}pix/$\tau${]}\tabularnewline
\hline 
\multirow{3}{*}{PointNet} & 8 & $3.17$\tabularnewline
\cline{2-3} 
 & 16 & $3.12$\tabularnewline
\cline{2-3} 
 & 32 & $3.14$\tabularnewline
\hline 
\multirow{3}{*}{EventNet} & 8 & $5.54$\tabularnewline
\cline{2-3} 
 & 16 & $3.94$\tabularnewline
\cline{2-3} 
 & 32 & $\textbf{3.11}$\tabularnewline
\hline 
\end{tabular}
\end{center}
\end{table}



